Salient Object Detection: A Benchmark

We extensively compare, qualitatively and quantitatively, 40 state-of-the-art models (28 salient object detection, 10 fixation prediction, 1 objectness, and 1 baseline) over 6 challenging datasets for the purpose of benchmarking salient object detection and segmentation methods. From the results obtained so far, our evaluation shows a consistent rapid progress over the last few years in terms of both accuracy and running time. The top contenders in this benchmark significantly outperform the models identified as the best in the previous benchmark conducted just two years ago. We find that the models designed specifically for salient object detection generally work better than models in closely related areas, which in turn provides a precise definition and suggests an appropriate treatment of this problem that distinguishes it from other problems. In particular, we analyze the influences of center bias and scene complexity in model performance, which, along with the hard cases for state-of-the-art models, provide useful hints towards constructing more challenging large scale datasets and better saliency models. Finally, we propose probable solutions for tackling several open problems such as evaluation scores and dataset bias, which also suggest future research directions in the rapidly-growing field of salient object detection.

==> ResNew/CutAdp.tex <==
\begin{tabular}{|l||c|c|c|c|c|c|} \hline
	\tabTitle \\	\hline \hline
	\textbf{ST}   & 0.604 & 0.580 & 0.394 & 0.577 & 0.825 & 0.690 \\
	\textbf{QCUT} & 0.656 & 0.625 & 0.454 & 0.647 & 0.843 & 0.738 \\
	\textbf{HDCT} & 0.576 & 0.571 & 0.378 & 0.572 & 0.807 & 0.669 \\
	\textbf{RBD}  & 0.610 & 0.566 & 0.403 & 0.580 & 0.821 & 0.680 \\
	\textbf{GR}   & 0.509 & 0.509 & 0.338 & 0.540 & 0.770 & 0.583 \\
	\textbf{MNP}  & 0.513 & 0.523 & 0.337 & 0.486 & 0.724 & 0.555 \\
	\textbf{UFO}  & 0.557 & 0.557 & 0.385 & 0.541 & 0.806 & 0.654 \\
	\textbf{MC}   & 0.623 & 0.603 & 0.420 & 0.603 & 0.824 & 0.704 \\
	\textbf{DSR}  & 0.622 & 0.604 & 0.421 & 0.614 & 0.824 & 0.717 \\
	\textbf{CHM}  & 0.588 & 0.591 & 0.368 & 0.586 & 0.804 & 0.684 \\
	\textbf{GC}   & 0.475 & 0.517 & 0.321 & 0.528 & 0.777 & 0.612 \\
	\textbf{LBI}  & 0.527 & 0.534 & 0.353 & 0.504 & 0.714 & 0.563 \\
	\textbf{PCA}  & 0.570 & 0.558 & 0.404 & 0.554 & 0.782 & 0.627 \\
	\textbf{DRFI} & 0.618 & 0.607 & 0.419 & 0.605 & 0.838 & 0.733 \\
	\textbf{GMR}  & 0.609 & 0.594 & 0.409 & 0.591 & 0.825 & 0.712 \\
	\textbf{HS}   & 0.561 & 0.549 & 0.358 & 0.565 & 0.800 & 0.659 \\
	\textbf{LMLC} & 0.508 & 0.519 & 0.302 & 0.493 & 0.772 & 0.600 \\
	\textbf{SF}   & 0.491 & 0.495 & 0.319 & 0.512 & 0.759 & 0.576 \\
	\textbf{FES}  & 0.606 & 0.575 & 0.411 & 0.555 & 0.753 & 0.655 \\
	\textbf{CB}   & 0.561 & 0.556 & 0.375 & 0.534 & 0.775 & 0.656 \\
	\textbf{SVO}  & 0.363 & 0.441 & 0.279 & 0.407 & 0.585 & \second{0.357} \\
	\textbf{SWD}  & 0.525 & 0.560 & 0.386 & 0.506 & 0.705 & 0.549 \\
	\textbf{HC}   & 0.385 & \second{0.401} & \third{0.257} & 0.380 & 0.663 & 0.441 \\
	\textbf{RC}   & 0.354 & 0.586 & 0.370 & 0.578 & 0.820 & 0.701 \\
	\textbf{SEG}  & \third{0.344} & 0.425 & 0.268 & 0.450 & 0.585 & 0.408 \\
	\textbf{MSS}  & 0.488 & 0.490 & 0.324 & 0.490 & 0.711 & 0.536 \\
	\textbf{CA}   & 0.475 & 0.494 & 0.330 & 0.458 & 0.679 & 0.494 \\
	\textbf{FT}   & 0.371 & \first{0.400} & \second{0.250} & 0.388 & 0.628 & 0.431 \\
	\textbf{AC}   & \first{0.281} & 0.431 & \first{0.199} & 0.383 & \first{0.566} & 0.410 \\
	\hline \hline
	\textbf{OBJ}  & 0.444 & 0.482 & 0.282 & 0.445 & 0.681 & 0.456 \\
	\hline \hline
	\textbf{BMS}  & 0.598 & 0.578 & 0.404 & 0.576 & 0.798 & 0.659 \\
	\textbf{COV}  & 0.605 & 0.587 & 0.427 & 0.579 & 0.755 & 0.677 \\
	\textbf{SS}   & 0.454 & 0.482 & 0.321 & 0.443 & 0.642 & 0.441 \\
	\textbf{SIM}  & 0.410 & 0.429 & 0.292 & 0.402 & 0.585 & 0.391 \\
	\textbf{SeR}  & 0.410 & \third{0.419} & 0.285 & 0.411 & 0.607 & 0.391 \\
	\textbf{SUN}  & \second{0.296} & 0.432 & 0.291 & \first{0.360} & 0.596 & \third{0.376} \\
	\textbf{SR}   & 0.444 & 0.457 & 0.270 & \second{0.363} & \second{0.569} & 0.385 \\
	\textbf{GB}   & 0.569 & 0.571 & 0.396 & 0.548 & 0.737 & 0.613 \\
	\textbf{AIM}  & 0.377 & 0.461 & 0.260 & \third{0.377} & \third{0.575} & \first{0.357} \\
	\textbf{IT}   & 0.456 & 0.437 & 0.283 & 0.449 & 0.586 & 0.414 \\
	\hline \hline
	\textbf{AVG}  & 0.537 & 0.569 & 0.367 & 0.514 & 0.692 & 0.627 \\
\hline
\end{tabular}


==> ResNew/MaxAdpScTDUTOMRON.tex <==
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &   ST& QCUT& HDCT&  RBD&   GR&  MNP&  UFO&   MC&  DSR&  CHM&   GC&  LBI&  PCA& DRFI&  GMR&   HS& LMLC&   SF&  FES&   CB\\\hline
	Max   & \third{0.631} & \first{0.683} & 0.609 & 0.630 & 0.599 & 0.467 & 0.545 & 0.627 & 0.626 & 0.604 & 0.535 & 0.482 & 0.554 & \second{0.665} & 0.610 & 0.616 & 0.521 & 0.519 & 0.520 & 0.542 \\
	AUC   & 0.895 & \third{0.897} & 0.869 & 0.894 & 0.846 & 0.835 & 0.839 & 0.887 & \second{0.899} & 0.890 & 0.796 & 0.854 & 0.887 & \first{0.933} & 0.853 & 0.860 & 0.817 & 0.803 & 0.848 & 0.831 \\
	MAE   & 0.182 & \first{0.119} & 0.164 & \third{0.144} & 0.259 & 0.272 & 0.173 & 0.186 & \second{0.139} & 0.152 & 0.197 & 0.249 & 0.206 & 0.155 & 0.189 & 0.227 & 0.277 & 0.183 & 0.156 & 0.257 \\
\hline
\end{tabular}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &  SVO&  SWD&   HC&   RC&  SEG&  MSS&   CA&   FT&   AC&  OBJ&  BMS&  COV&   SS&  SIM&  SeR&  SUN&   SR&   GB&  AIM&   IT\\\hline
	Max   & 0.557 & 0.478 & 0.382 & 0.599 & 0.516 & 0.476 & 0.435 & 0.381 & 0.354 & 0.481 & 0.573 & 0.486 & 0.396 & 0.358 & 0.385 & 0.321 & 0.298 & 0.507 & 0.361 & 0.378 \\
	AUC   & 0.866 & 0.843 & 0.733 & 0.859 & 0.825 & 0.817 & 0.815 & 0.682 & 0.721 & 0.822 & 0.856 & 0.864 & 0.784 & 0.783 & 0.786 & 0.708 & 0.688 & 0.857 & 0.768 & 0.636 \\
	MAE   & 0.409 & 0.310 & 0.310 & 0.189 & 0.337 & 0.177 & 0.254 & 0.250 & 0.190 & 0.323 & 0.175 & 0.156 & 0.277 & 0.429 & 0.352 & 0.349 & 0.181 & 0.240 & 0.322 & 0.198 \\
\hline
\end{tabular}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &  AVG&     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     \\\hline
	Max   & 0.406 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
	AUC   & 0.814 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
	MAE   & 0.288 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
\hline
\end{tabular}


==> ResNew/MaxAdpScTECSSD.tex <==
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &   ST& QCUT& HDCT&  RBD&   GR&  MNP&  UFO&   MC&  DSR&  CHM&   GC&  LBI&  PCA& DRFI&  GMR&   HS& LMLC&   SF&  FES&   CB\\\hline
	Max   & \third{0.752} & \second{0.779} & 0.705 & 0.718 & 0.664 & 0.568 & 0.701 & 0.742 & 0.737 & 0.722 & 0.641 & 0.586 & 0.646 & \first{0.787} & 0.740 & 0.731 & 0.659 & 0.619 & 0.645 & 0.717 \\
	AUC   & \third{0.914} & 0.909 & 0.866 & 0.894 & 0.831 & 0.820 & 0.875 & 0.910 & \second{0.914} & 0.903 & 0.805 & 0.842 & 0.876 & \first{0.944} & 0.889 & 0.883 & 0.849 & 0.817 & 0.860 & 0.875 \\
	MAE   & 0.193 & \second{0.171} & 0.199 & 0.173 & 0.285 & 0.307 & 0.207 & 0.204 & \third{0.173} & 0.195 & 0.214 & 0.280 & 0.248 & \first{0.166} & 0.189 & 0.228 & 0.260 & 0.230 & 0.215 & 0.241 \\
\hline
\end{tabular}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &  SVO&  SWD&   HC&   RC&  SEG&  MSS&   CA&   FT&   AC&  OBJ&  BMS&  COV&   SS&  SIM&  SeR&  SUN&   SR&   GB&  AIM&   IT\\\hline
	Max   & 0.639 & 0.624 & 0.460 & 0.741 & 0.568 & 0.530 & 0.515 & 0.434 & 0.411 & 0.574 & 0.683 & 0.641 & 0.467 & 0.433 & 0.419 & 0.388 & 0.381 & 0.624 & 0.449 & 0.407 \\
	AUC   & 0.857 & 0.857 & 0.704 & 0.892 & 0.808 & 0.779 & 0.784 & 0.661 & 0.668 & 0.818 & 0.865 & 0.879 & 0.725 & 0.734 & 0.695 & 0.623 & 0.633 & 0.865 & 0.730 & 0.577 \\
	MAE   & 0.404 & 0.318 & 0.331 & 0.187 & 0.342 & 0.245 & 0.310 & 0.291 & 0.265 & 0.337 & 0.216 & 0.217 & 0.344 & 0.433 & 0.404 & 0.396 & 0.266 & 0.263 & 0.339 & 0.273 \\
\hline
\end{tabular}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &  AVG&     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     \\\hline
	Max   & 0.597 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
	AUC   & 0.863 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
	MAE   & 0.276 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
\hline
\end{tabular}


==> ResNew/MaxAdpScTJuddDB.tex <==
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &   ST& QCUT& HDCT&  RBD&   GR&  MNP&  UFO&   MC&  DSR&  CHM&   GC&  LBI&  PCA& DRFI&  GMR&   HS& LMLC&   SF&  FES&   CB\\\hline
	Max   & 0.455 & \first{0.509} & 0.412 & 0.457 & 0.418 & 0.367 & 0.432 & \third{0.460} & 0.454 & 0.417 & 0.384 & 0.371 & 0.432 & \second{0.475} & 0.454 & 0.442 & 0.375 & 0.373 & 0.424 & 0.444 \\
	AUC   & 0.806 & \second{0.831} & 0.771 & \third{0.826} & 0.747 & 0.768 & 0.775 & 0.823 & 0.826 & 0.797 & 0.702 & 0.792 & 0.804 & \first{0.851} & 0.781 & 0.775 & 0.724 & 0.711 & 0.805 & 0.760 \\
	MAE   & 0.240 & \first{0.178} & 0.209 & 0.212 & 0.311 & 0.286 & 0.216 & 0.231 & 0.196 & 0.226 & 0.258 & 0.273 & \second{0.181} & 0.213 & 0.243 & 0.282 & 0.303 & 0.218 & 0.184 & 0.287 \\
\hline
\end{tabular}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &  SVO&  SWD&   HC&   RC&  SEG&  MSS&   CA&   FT&   AC&  OBJ&  BMS&  COV&   SS&  SIM&  SeR&  SUN&   SR&   GB&  AIM&   IT\\\hline
	Max   & 0.414 & 0.434 & 0.286 & 0.431 & 0.376 & 0.341 & 0.353 & 0.278 & 0.227 & 0.368 & 0.434 & 0.429 & 0.344 & 0.295 & 0.316 & 0.303 & 0.279 & 0.419 & 0.317 & 0.297 \\
	AUC   & 0.784 & 0.812 & 0.626 & 0.775 & 0.747 & 0.726 & 0.774 & 0.593 & 0.548 & 0.750 & 0.788 & 0.826 & 0.754 & 0.727 & 0.746 & 0.674 & 0.676 & 0.815 & 0.719 & 0.586 \\
	MAE   & 0.422 & 0.292 & 0.348 & 0.270 & 0.354 & 0.204 & 0.282 & 0.267 & 0.239 & 0.359 & 0.233 & \third{0.182} & 0.301 & 0.412 & 0.379 & 0.319 & 0.200 & 0.261 & 0.331 & 0.200 \\
\hline
\end{tabular}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &  AVG&     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     \\\hline
	Max   & 0.392 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
	AUC   & 0.797 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
	MAE   & 0.343 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
\hline
\end{tabular}


==> ResNew/MaxAdpScTMSRA10K.tex <==
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &   ST& QCUT& HDCT&  RBD&   GR&  MNP&  UFO&   MC&  DSR&  CHM&   GC&  LBI&  PCA& DRFI&  GMR&   HS& LMLC&   SF&  FES&   CB\\\hline
	Max   & \third{0.868} & \second{0.874} & 0.837 & 0.856 & 0.816 & 0.668 & 0.842 & 0.847 & 0.835 & 0.825 & 0.794 & 0.696 & 0.782 & \first{0.881} & 0.847 & 0.845 & 0.801 & 0.779 & 0.717 & 0.815 \\
	AUC   & \second{0.961} & 0.956 & 0.941 & 0.955 & 0.925 & 0.895 & 0.938 & 0.951 & \third{0.959} & 0.952 & 0.912 & 0.910 & 0.941 & \first{0.978} & 0.944 & 0.933 & 0.936 & 0.905 & 0.898 & 0.927 \\
	MAE   & 0.122 & \second{0.118} & 0.143 & \first{0.108} & 0.198 & 0.229 & 0.150 & 0.145 & 0.121 & 0.142 & 0.139 & 0.224 & 0.185 & \third{0.118} & 0.126 & 0.149 & 0.163 & 0.175 & 0.185 & 0.178 \\
\hline
\end{tabular}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &  SVO&  SWD&   HC&   RC&  SEG&  MSS&   CA&   FT&   AC&  OBJ&  BMS&  COV&   SS&  SIM&  SeR&  SUN&   SR&   GB&  AIM&   IT\\\hline
	Max   & 0.789 & 0.689 & 0.677 & 0.844 & 0.697 & 0.696 & 0.621 & 0.635 & 0.520 & 0.718 & 0.805 & 0.667 & 0.572 & 0.498 & 0.542 & 0.505 & 0.473 & 0.688 & 0.555 & 0.471 \\
	AUC   & 0.930 & 0.901 & 0.867 & 0.936 & 0.882 & 0.875 & 0.872 & 0.790 & 0.756 & 0.907 & 0.929 & 0.904 & 0.823 & 0.808 & 0.813 & 0.778 & 0.736 & 0.902 & 0.833 & 0.640 \\
	MAE   & 0.331 & 0.267 & 0.215 & 0.137 & 0.298 & 0.203 & 0.237 & 0.235 & 0.227 & 0.262 & 0.151 & 0.197 & 0.266 & 0.388 & 0.310 & 0.306 & 0.232 & 0.222 & 0.286 & 0.213 \\
\hline
\end{tabular}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &  AVG&     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     \\\hline
	Max   & 0.580 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
	AUC   & 0.857 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
	MAE   & 0.260 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
\hline
\end{tabular}


==> ResNew/MaxAdpScTPASCAL-S.tex <==
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &   ST& QCUT& HDCT&  RBD&   GR&  MNP&  UFO&   MC&  DSR&  CHM&   GC&  LBI&  PCA& DRFI&  GMR&   HS& LMLC&   SF&  FES&   CB\\\hline
	Max   & 0.660 & \first{0.695} & 0.604 & 0.652 & 0.596 & 0.522 & 0.606 & \third{0.661} & 0.646 & 0.631 & 0.535 & 0.538 & 0.593 & \second{0.679} & 0.643 & 0.637 & 0.555 & 0.544 & 0.619 & 0.623 \\
	AUC   & 0.868 & 0.870 & 0.815 & 0.867 & 0.794 & 0.807 & 0.825 & \second{0.873} & \third{0.873} & 0.864 & 0.728 & 0.828 & 0.848 & \first{0.897} & 0.829 & 0.840 & 0.800 & 0.762 & 0.854 & 0.818 \\
	MAE   & 0.224 & \first{0.195} & 0.229 & \second{0.199} & 0.299 & 0.298 & 0.245 & 0.230 & \third{0.204} & 0.222 & 0.265 & 0.281 & 0.245 & 0.221 & 0.233 & 0.262 & 0.284 & 0.253 & 0.218 & 0.272 \\
\hline
\end{tabular}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &  SVO&  SWD&   HC&   RC&  SEG&  MSS&   CA&   FT&   AC&  OBJ&  BMS&  COV&   SS&  SIM&  SeR&  SUN&   SR&   GB&  AIM&   IT\\\hline
	Max   & 0.586 & 0.577 & 0.423 & 0.466 & 0.534 & 0.503 & 0.489 & 0.408 & 0.326 & 0.544 & 0.617 & 0.589 & 0.469 & 0.434 & 0.433 & 0.359 & 0.447 & 0.581 & 0.450 & 0.414 \\
	AUC   & 0.826 & 0.835 & 0.669 & 0.713 & 0.787 & 0.766 & 0.782 & 0.629 & 0.565 & 0.811 & 0.834 & 0.856 & 0.752 & 0.756 & 0.736 & 0.588 & 0.745 & 0.843 & 0.753 & 0.621 \\
	MAE   & 0.392 & 0.315 & 0.354 & 0.304 & 0.350 & 0.251 & 0.299 & 0.307 & 0.286 & 0.334 & 0.225 & 0.226 & 0.315 & 0.414 & 0.371 & 0.467 & 0.291 & 0.270 & 0.337 & 0.240 \\
\hline
\end{tabular}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &  AVG&     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     \\\hline
	Max   & 0.549 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
	AUC   & 0.835 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
	MAE   & 0.320 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
\hline
\end{tabular}


==> ResNew/MaxAdpScTSED2.tex <==
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &   ST& QCUT& HDCT&  RBD&   GR&  MNP&  UFO&   MC&  DSR&  CHM&   GC&  LBI&  PCA& DRFI&  GMR&   HS& LMLC&   SF&  FES&   CB\\\hline
	Max   & 0.818 & 0.810 & \third{0.822} & \first{0.837} & 0.798 & 0.621 & 0.742 & 0.779 & 0.794 & 0.750 & 0.729 & 0.692 & 0.754 & \second{0.831} & 0.773 & 0.811 & 0.653 & 0.764 & 0.617 & 0.730 \\
	AUC   & \second{0.922} & 0.860 & 0.898 & 0.899 & 0.854 & 0.888 & 0.845 & 0.877 & \third{0.915} & 0.831 & 0.846 & 0.896 & 0.911 & \first{0.944} & 0.862 & 0.858 & 0.826 & 0.871 & 0.838 & 0.839 \\
	MAE   & 0.145 & 0.148 & 0.162 & \second{0.130} & 0.189 & 0.215 & 0.180 & 0.182 & \third{0.140} & 0.168 & 0.185 & 0.207 & 0.200 & \first{0.130} & 0.163 & 0.157 & 0.269 & 0.180 & 0.196 & 0.195 \\
\hline
\end{tabular}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &  SVO&  SWD&   HC&   RC&  SEG&  MSS&   CA&   FT&   AC&  OBJ&  BMS&  COV&   SS&  SIM&  SeR&  SUN&   SR&   GB&  AIM&   IT\\\hline
	Max   & 0.744 & 0.548 & 0.736 & 0.774 & 0.704 & 0.743 & 0.591 & 0.715 & 0.684 & 0.685 & 0.713 & 0.518 & 0.533 & 0.498 & 0.521 & 0.504 & 0.504 & 0.571 & 0.541 & 0.579 \\
	AUC   & 0.875 & 0.845 & 0.880 & 0.852 & 0.796 & 0.871 & 0.853 & 0.820 & 0.831 & 0.870 & 0.852 & 0.833 & 0.826 & 0.833 & 0.835 & 0.789 & 0.769 & 0.839 & 0.846 & 0.682 \\
	MAE   & 0.348 & 0.296 & 0.193 & 0.148 & 0.312 & 0.192 & 0.229 & 0.206 & 0.206 & 0.269 & 0.184 & 0.210 & 0.266 & 0.384 & 0.290 & 0.307 & 0.220 & 0.242 & 0.262 & 0.245 \\
\hline
\end{tabular}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &  AVG&     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     \\\hline
	Max   & 0.388 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
	AUC   & 0.736 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
	MAE   & 0.405 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
\hline
\end{tabular}


==> ResNew/MaxAdpScTTHUR15K.tex <==
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &   ST& QCUT& HDCT&  RBD&   GR&  MNP&  UFO&   MC&  DSR&  CHM&   GC&  LBI&  PCA& DRFI&  GMR&   HS& LMLC&   SF&  FES&   CB\\\hline
	Max   & \third{0.631} & \second{0.651} & 0.602 & 0.596 & 0.551 & 0.495 & 0.579 & 0.610 & 0.611 & 0.612 & 0.533 & 0.519 & 0.544 & \first{0.670} & 0.597 & 0.585 & 0.540 & 0.500 & 0.547 & 0.581 \\
	AUC   & \second{0.911} & 0.907 & 0.878 & 0.887 & 0.829 & 0.854 & 0.853 & 0.895 & 0.902 & \third{0.910} & 0.803 & 0.876 & 0.885 & \first{0.938} & 0.856 & 0.853 & 0.853 & 0.799 & 0.867 & 0.870 \\
	MAE   & 0.179 & \first{0.128} & 0.177 & 0.150 & 0.256 & 0.255 & 0.165 & 0.184 & \second{0.142} & 0.153 & 0.192 & 0.239 & 0.198 & \third{0.150} & 0.181 & 0.218 & 0.246 & 0.184 & 0.155 & 0.227 \\
\hline
\end{tabular}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &  SVO&  SWD&   HC&   RC&  SEG&  MSS&   CA&   FT&   AC&  OBJ&  BMS&  COV&   SS&  SIM&  SeR&  SUN&   SR&   GB&  AIM&   IT\\\hline
	Max   & 0.554 & 0.528 & 0.386 & 0.610 & 0.500 & 0.478 & 0.458 & 0.386 & 0.382 & 0.498 & 0.568 & 0.510 & 0.415 & 0.372 & 0.374 & 0.387 & 0.374 & 0.526 & 0.427 & 0.373 \\
	AUC   & 0.865 & 0.873 & 0.735 & 0.896 & 0.818 & 0.813 & 0.830 & 0.684 & 0.707 & 0.839 & 0.879 & 0.883 & 0.792 & 0.797 & 0.778 & 0.746 & 0.741 & 0.882 & 0.814 & 0.623 \\
	MAE   & 0.382 & 0.288 & 0.291 & 0.168 & 0.336 & 0.178 & 0.248 & 0.241 & 0.195 & 0.306 & 0.181 & 0.155 & 0.267 & 0.414 & 0.345 & 0.310 & 0.175 & 0.229 & 0.298 & 0.199 \\
\hline
\end{tabular}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method &  AVG&     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     \\\hline
	Max   & 0.458 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
	AUC   & 0.849 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
	MAE   & 0.248 &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      \\
\hline
\end{tabular}


==> ResNew/MaxF.tex <==
\begin{tabular}{|l||c|c|c|c|c|c|} \hline
	\tabTitle \\	\hline \hline
	\textbf{ST}   & 0.660 & \third{0.631} & 0.455 & \third{0.631} & \third{0.868} & \third{0.752} \\
	\textbf{QCUT} & \first{0.695} & \second{0.651} & \first{0.509} & \first{0.683} & \second{0.874} & \second{0.779} \\
	\textbf{HDCT} & 0.604 & 0.602 & 0.412 & 0.609 & 0.837 & 0.705 \\
	\textbf{RBD}  & 0.652 & 0.596 & 0.457 & 0.630 & 0.856 & 0.718 \\
	\textbf{GR}   & 0.596 & 0.551 & 0.418 & 0.599 & 0.816 & 0.664 \\
	\textbf{MNP}  & 0.522 & 0.495 & 0.367 & 0.467 & 0.668 & 0.568 \\
	\textbf{UFO}  & 0.606 & 0.579 & 0.432 & 0.545 & 0.842 & 0.701 \\
	\textbf{MC}   & \third{0.661} & 0.610 & \third{0.460} & 0.627 & 0.847 & 0.742 \\
	\textbf{DSR}  & 0.646 & 0.611 & 0.454 & 0.626 & 0.835 & 0.737 \\
	\textbf{CHM}  & 0.631 & 0.612 & 0.417 & 0.604 & 0.825 & 0.722 \\
	\textbf{GC}   & 0.535 & 0.533 & 0.384 & 0.535 & 0.794 & 0.641 \\
	\textbf{LBI}  & 0.538 & 0.519 & 0.371 & 0.482 & 0.696 & 0.586 \\
	\textbf{PCA}  & 0.593 & 0.544 & 0.432 & 0.554 & 0.782 & 0.646 \\
	\textbf{DRFI} & \second{0.679} & \first{0.670} & \second{0.475} & \second{0.665} & \first{0.881} & \first{0.787} \\
	\textbf{GMR}  & 0.643 & 0.597 & 0.454 & 0.610 & 0.847 & 0.740 \\
	\textbf{HS}   & 0.637 & 0.585 & 0.442 & 0.616 & 0.845 & 0.731 \\
	\textbf{LMLC} & 0.555 & 0.540 & 0.375 & 0.521 & 0.801 & 0.659 \\
	\textbf{SF}   & 0.544 & 0.500 & 0.373 & 0.519 & 0.779 & 0.619 \\
	\textbf{FES}  & 0.619 & 0.547 & 0.424 & 0.520 & 0.717 & 0.645 \\
	\textbf{CB}   & 0.623 & 0.581 & 0.444 & 0.542 & 0.815 & 0.717 \\
	\textbf{SVO}  & 0.586 & 0.554 & 0.414 & 0.557 & 0.789 & 0.639 \\
	\textbf{SWD}  & 0.577 & 0.528 & 0.434 & 0.478 & 0.689 & 0.624 \\
	\textbf{HC}   & 0.423 & 0.386 & 0.286 & 0.382 & 0.677 & 0.460 \\
	\textbf{RC}   & 0.466 & 0.610 & 0.431 & 0.599 & 0.844 & 0.741 \\
	\textbf{SEG}  & 0.534 & 0.500 & 0.376 & 0.516 & 0.697 & 0.568 \\
	\textbf{MSS}  & 0.503 & 0.478 & 0.341 & 0.476 & 0.696 & 0.530 \\
	\textbf{CA}   & 0.489 & 0.458 & 0.353 & 0.435 & 0.621 & 0.515 \\
	\textbf{FT}   & 0.408 & 0.386 & 0.278 & 0.381 & 0.635 & 0.434 \\
	\textbf{AC}   & 0.326 & 0.382 & 0.227 & 0.354 & 0.520 & 0.411 \\
	\hline \hline
	\textbf{OBJ}  & 0.544 & 0.498 & 0.368 & 0.481 & 0.718 & 0.574 \\
	\hline \hline
	\textbf{BMS}  & 0.617 & 0.568 & 0.434 & 0.573 & 0.805 & 0.683 \\
	\textbf{COV}  & 0.589 & 0.510 & 0.429 & 0.486 & 0.667 & 0.641 \\
	\textbf{SS}   & 0.469 & 0.415 & 0.344 & 0.396 & 0.572 & 0.467 \\
	\textbf{SIM}  & 0.434 & 0.372 & 0.295 & 0.358 & 0.498 & 0.433 \\
	\textbf{SeR}  & 0.433 & 0.374 & 0.316 & 0.385 & 0.542 & 0.419 \\
	\textbf{SUN}  & 0.359 & 0.387 & 0.303 & 0.321 & 0.505 & 0.388 \\
	\textbf{SR}   & 0.447 & 0.374 & 0.279 & 0.298 & 0.473 & 0.381 \\
	\textbf{GB}   & 0.581 & 0.526 & 0.419 & 0.507 & 0.688 & 0.624 \\
	\textbf{AIM}  & 0.450 & 0.427 & 0.317 & 0.361 & 0.555 & 0.449 \\
	\textbf{IT}   & 0.414 & 0.373 & 0.297 & 0.378 & 0.471 & 0.407 \\
	\hline \hline
	\textbf{AVG}  & 0.549 & 0.458 & 0.392 & 0.406 & 0.580 & 0.597 \\
\hline
\end{tabular}


==> ResNew/MeanF.tex <==
\begin{tabular}{|l||c|c|c|c|c|c|} \hline
	\tabTitle \\	\hline \hline
	\textbf{ST}   & \third{0.561} & 0.541 & 0.394 & 0.536 & 0.762 & 0.638 \\
	\textbf{QCUT} & 0.551 & \second{0.555} & \first{0.430} & \first{0.600} & 0.751 & 0.632 \\
	\textbf{HDCT} & 0.494 & 0.500 & 0.351 & 0.505 & 0.713 & 0.590 \\
	\textbf{RBD}  & \first{0.568} & 0.526 & \second{0.415} & 0.551 & \first{0.768} & 0.622 \\
	\textbf{GR}   & 0.470 & 0.444 & 0.343 & 0.471 & 0.666 & 0.518 \\
	\textbf{MNP}  & 0.413 & 0.390 & 0.303 & 0.370 & 0.512 & 0.433 \\
	\textbf{UFO}  & 0.465 & 0.468 & 0.335 & 0.451 & 0.670 & 0.533 \\
	\textbf{MC}   & 0.546 & 0.515 & 0.392 & 0.529 & 0.733 & 0.611 \\
	\textbf{DSR}  & 0.560 & \third{0.551} & 0.402 & \second{0.560} & \third{0.765} & \second{0.645} \\
	\textbf{CHM}  & 0.491 & 0.508 & 0.336 & 0.512 & 0.700 & 0.576 \\
	\textbf{GC}   & 0.492 & 0.488 & 0.357 & 0.489 & 0.729 & 0.577 \\
	\textbf{LBI}  & 0.418 & 0.402 & 0.299 & 0.371 & 0.548 & 0.442 \\
	\textbf{PCA}  & 0.430 & 0.413 & 0.330 & 0.429 & 0.566 & 0.465 \\
	\textbf{DRFI} & \second{0.561} & \first{0.573} & 0.387 & \third{0.555} & 0.761 & \first{0.667} \\
	\textbf{GMR}  & 0.559 & 0.533 & \third{0.403} & 0.537 & \second{0.766} & \third{0.643} \\
	\textbf{HS}   & 0.550 & 0.516 & 0.384 & 0.520 & 0.752 & 0.623 \\
	\textbf{LMLC} & 0.493 & 0.460 & 0.340 & 0.417 & 0.714 & 0.562 \\
	\textbf{SF}   & 0.358 & 0.365 & 0.244 & 0.401 & 0.556 & 0.414 \\
	\textbf{FES}  & 0.408 & 0.390 & 0.304 & 0.370 & 0.471 & 0.421 \\
	\textbf{CB}   & 0.508 & 0.474 & 0.360 & 0.433 & 0.686 & 0.571 \\
	\textbf{SVO}  & 0.431 & 0.382 & 0.314 & 0.361 & 0.540 & 0.443 \\
	\textbf{SWD}  & 0.413 & 0.371 & 0.296 & 0.338 & 0.478 & 0.443 \\
	\textbf{HC}   & 0.372 & 0.347 & 0.260 & 0.331 & 0.597 & 0.401 \\
	\textbf{RC}   & 0.383 & 0.530 & 0.360 & 0.506 & 0.729 & 0.637 \\
	\textbf{SEG}  & 0.399 & 0.371 & 0.302 & 0.378 & 0.491 & 0.441 \\
	\textbf{MSS}  & 0.261 & 0.280 & 0.191 & 0.288 & 0.389 & 0.290 \\
	\textbf{CA}   & 0.360 & 0.346 & 0.280 & 0.328 & 0.455 & 0.378 \\
	\textbf{FT}   & 0.261 & 0.268 & 0.187 & 0.268 & 0.420 & 0.286 \\
	\textbf{AC}   & 0.140 & 0.207 & 0.115 & 0.188 & 0.171 & 0.191 \\
	\hline \hline
	\textbf{OBJ}  & 0.419 & 0.373 & 0.295 & 0.353 & 0.535 & 0.434 \\
	\hline \hline
	\textbf{BMS}  & 0.530 & 0.485 & 0.363 & 0.503 & 0.693 & 0.582 \\
	\textbf{COV}  & 0.349 & 0.333 & 0.291 & 0.334 & 0.363 & 0.371 \\
	\textbf{SS}   & 0.329 & 0.304 & 0.263 & 0.295 & 0.388 & 0.331 \\
	\textbf{SIM}  & 0.338 & 0.269 & 0.231 & 0.258 & 0.365 & 0.332 \\
	\textbf{SeR}  & 0.369 & 0.305 & 0.271 & 0.296 & 0.436 & 0.346 \\
	\textbf{SUN}  & 0.338 & 0.261 & 0.194 & 0.227 & 0.337 & 0.270 \\
	\textbf{SR}   & 0.301 & 0.162 & 0.117 & 0.137 & 0.165 & 0.143 \\
	\textbf{GB}   & 0.408 & 0.374 & 0.304 & 0.361 & 0.470 & 0.438 \\
	\textbf{AIM}  & 0.314 & 0.289 & 0.218 & 0.246 & 0.390 & 0.303 \\
	\textbf{IT}   & 0.315 & 0.195 & 0.146 & 0.216 & 0.351 & 0.177 \\
	\hline \hline
	\textbf{AVG}  & 0.438 & 0.358 & 0.313 & 0.325 & 0.475 & 0.484 \\
\hline
\end{tabular}


==> ResNew/SalCut.tex <==
\begin{tabular}{|l||c|c|c|c|c|c|} \hline
	\tabTitle \\	\hline \hline
	\textbf{ST}   & \second{0.675} & 0.648 & \third{0.459} & 0.635 & \second{0.896} & \third{0.777} \\
	\textbf{QCUT} & 0.614 & 0.620 & \first{0.480} & \third{0.647} & 0.843 & 0.747 \\
	\textbf{HDCT} & 0.613 & 0.636 & 0.422 & 0.643 & 0.877 & 0.740 \\
	\textbf{RBD}  & 0.670 & 0.618 & \second{0.461} & \second{0.647} & \third{0.884} & 0.757 \\
	\textbf{GR}   & 0.607 & 0.546 & 0.378 & 0.580 & 0.830 & 0.677 \\
	\textbf{MNP}  & 0.634 & 0.603 & 0.405 & 0.576 & 0.822 & 0.709 \\
	\textbf{UFO}  & 0.624 & 0.610 & 0.433 & 0.593 & 0.862 & 0.739 \\
	\textbf{MC}   & \third{0.674} & 0.600 & 0.434 & 0.615 & 0.855 & 0.745 \\
	\textbf{DSR}  & 0.651 & 0.597 & 0.410 & 0.593 & 0.833 & 0.703 \\
	\textbf{CHM}  & 0.638 & 0.643 & 0.424 & 0.637 & 0.857 & 0.735 \\
	\textbf{GC}   & 0.556 & 0.497 & 0.342 & 0.506 & 0.780 & 0.593 \\
	\textbf{LBI}  & 0.632 & 0.618 & 0.416 & 0.609 & 0.857 & 0.738 \\
	\textbf{PCA}  & 0.636 & 0.601 & 0.368 & 0.624 & 0.845 & 0.720 \\
	\textbf{DRFI} & \first{0.693} & \first{0.674} & 0.447 & \first{0.669} & \first{0.905} & \first{0.801} \\
	\textbf{GMR}  & 0.656 & 0.579 & 0.432 & 0.591 & 0.839 & 0.736 \\
	\textbf{HS}   & 0.653 & 0.602 & 0.428 & 0.616 & 0.870 & 0.769 \\
	\textbf{LMLC} & 0.617 & 0.588 & 0.397 & 0.551 & 0.860 & 0.735 \\
	\textbf{SF}   & 0.463 & 0.342 & 0.219 & 0.377 & 0.573 & 0.378 \\
	\textbf{FES}  & 0.532 & 0.426 & 0.333 & 0.380 & 0.534 & 0.467 \\
	\textbf{CB}   & 0.637 & 0.615 & 0.435 & 0.593 & 0.857 & 0.761 \\
	\textbf{SVO}  & 0.624 & 0.609 & 0.419 & 0.609 & 0.863 & 0.737 \\
	\textbf{SWD}  & 0.646 & \third{0.649} & 0.454 & 0.613 & 0.871 & \second{0.781} \\
	\textbf{HC}   & 0.468 & 0.436 & 0.280 & 0.435 & 0.740 & 0.499 \\
	\textbf{RC}   & 0.475 & 0.639 & 0.425 & 0.621 & 0.875 & 0.776 \\
	\textbf{SEG}  & 0.631 & 0.580 & 0.393 & 0.562 & 0.812 & 0.715 \\
	\textbf{MSS}  & 0.399 & 0.200 & 0.089 & 0.193 & 0.362 & 0.203 \\
	\textbf{CA}   & 0.589 & 0.557 & 0.394 & 0.532 & 0.748 & 0.625 \\
	\textbf{FT}   & 0.359 & 0.238 & 0.132 & 0.259 & 0.472 & 0.257 \\
	\textbf{AC}   & 0.265 & 0.068 & 0.049 & 0.040 & 0.014 & 0.038 \\
	\hline \hline
	\textbf{OBJ}  & 0.601 & 0.593 & 0.413 & 0.578 & 0.840 & 0.698 \\
	\hline \hline
	\textbf{BMS}  & 0.624 & 0.594 & 0.416 & 0.580 & 0.822 & 0.690 \\
	\textbf{COV}  & 0.535 & 0.398 & 0.315 & 0.373 & 0.394 & 0.413 \\
	\textbf{SS}   & 0.555 & 0.523 & 0.397 & 0.502 & 0.675 & 0.574 \\
	\textbf{SIM}  & 0.602 & 0.568 & 0.384 & 0.539 & 0.794 & 0.672 \\
	\textbf{SeR}  & 0.570 & 0.536 & 0.388 & 0.532 & 0.755 & 0.596 \\
	\textbf{SUN}  & 0.472 & 0.486 & 0.285 & 0.445 & 0.670 & 0.478 \\
	\textbf{SR}   & 0.498 & 0.002 & 0.001 & 0.000 & 0.001 & 0.001 \\
	\textbf{GB}   & 0.653 & \second{0.650} & 0.455 & 0.638 & 0.837 & 0.765 \\
	\textbf{AIM}  & 0.597 & 0.559 & 0.360 & 0.495 & 0.750 & 0.571 \\
	\textbf{IT}   & 0.255 & 0.005 & 0.000 & 0.005 & 0.158 & 0.003 \\
	\hline \hline
	\textbf{AVG}  & 0.582 & 0.620 & 0.411 & 0.534 & 0.779 & 0.756 \\
\hline
\end{tabular}


==> Results/AUC.tex <==
\begin{tabular}{|l||c|c|c|c|c|c|} \hline
	\tabTitle \\	\hline \hline
	\textbf{HDCT} & .878 & .771 & .869 & .898 & .941 & .866 \\
	\textbf{RBD}  & .887 & \second{.826} & \third{.894} & .899 & \third{.955} & .894 \\
	\textbf{GR}   & .829 & .747 & .846 & .854 & .925 & .831 \\
	\textbf{MNP}  & .854 & .768 & .835 & .888 & .895 & .820 \\
	\textbf{UFO}  & .853 & .775 & .839 & .845 & .938 & .875 \\
	\textbf{MC}   & .895 & .823 & .887 & .877 & .951 & \third{.910} \\
	\textbf{DSR}  & \third{.902} & .826 & \second{.899} & \second{.915} & \second{.959} & \second{.914} \\
	\textbf{CHM}  & \second{.910} & .797 & .890 & .831 & .952 & .903 \\
	\textbf{GC}   & .803 & .702 & .796 & .846 & .912 & .805 \\
	\textbf{LBI}  & .876 & .792 & .854 & .896 & .910 & .842 \\
	\textbf{PCA}  & .885 & .804 & .887 & \third{.911} & .941 & .876 \\
	\textbf{DRFI} & \first{.938} & \first{.851} & \first{.933} & \first{.944} & \first{.978} & \first{.944} \\
	\textbf{GMR}  & .856 & .781 & .853 & .862 & .944 & .889 \\
	\textbf{HS}   & .853 & .775 & .860 & .858 & .933 & .883 \\
	\textbf{LMLC} & .853 & .724 & .817 & .826 & .936 & .849 \\
	\textbf{SF}   & .799 & .711 & .803 & .871 & .905 & .817 \\
	\textbf{FES}  & .867 & .805 & .848 & .838 & .898 & .860 \\
	\textbf{CB}   & .870 & .760 & .831 & .839 & .927 & .875 \\
	\textbf{SVO}  & .865 & .784 & .866 & .875 & .930 & .857 \\
	\textbf{SWD}  & .873 & .812 & .843 & .845 & .901 & .857 \\
	\textbf{HC}   & .735 & .626 & .733 & .880 & .867 & .704 \\
	\textbf{RC}   & .896 & .775 & .859 & .852 & .936 & .892 \\
	\textbf{SEG}  & .818 & .747 & .825 & .796 & .882 & .808 \\
	\textbf{MSS}  & .813 & .726 & .817 & .871 & .875 & .779 \\
	\textbf{CA}   & .830 & .774 & .815 & .853 & .872 & .784 \\
	\textbf{FT}   & .684 & .593 & .682 & .820 & .790 & .661 \\
	\textbf{AC}   & .740 & .548 & .721 & .831 & .756 & .668 \\
	\textbf{LC}   & .696 & .586 & .654 & .827 & .771 & .627 \\
	\hline \hline
	\textbf{OBJ}  & .839 & .750 & .822 & .870 & .907 & .818 \\
	\hline \hline
	\textbf{BMS}  & .879 & .788 & .856 & .852 & .929 & .865 \\
	\textbf{COV}  & .883 & \third{.826} & .864 & .833 & .904 & .879 \\
	\textbf{SS}   & .792 & .754 & .784 & .826 & .823 & .725 \\
	\textbf{SIM}  & .797 & .727 & .783 & .833 & .808 & .734 \\
	\textbf{SeR}  & .778 & .746 & .786 & .835 & .813 & .695 \\
	\textbf{SUN}  & .746 & .674 & .708 & .789 & .778 & .623 \\
	\textbf{SR}   & .741 & .676 & .688 & .769 & .736 & .633 \\
	\textbf{GB}   & .882 & .815 & .857 & .839 & .902 & .865 \\
	\textbf{AIM}  & .814 & .719 & .768 & .846 & .833 & .730 \\
	\textbf{IT}   & .623 & .586 & .636 & .682 & .640 & .577 \\
	\hline \hline
	\textbf{AAM}  & .849 & .797 & .814 & .736 & .857 & .863 \\
\hline
\end{tabular}


==> Results/FixAdpSc.tex <==
\begin{tabular}{|l||ccc|ccc|ccc|ccc|ccc|ccc|} \hline
	\tabTitle \\	\hline \hline
	\textbf{HDCT} & .602 & .571 & .636 & .412 & .378 & .422 & .609 & .572 & \third{.643} & \third{.822} & .802 & \third{.758} & .837 & .807 & \third{.877} & .705 & .669 & .740 \\
	\textbf{RBD}  & .596 & .566 & .618 & \third{.457} & .403 & \first{.461} & \second{.630} & .580 & \second{.647} & \first{.837} & \second{.825} & .750 & \second{.856} & .821 & \second{.884} & .718 & .680 & .757 \\
	\textbf{GR}   & .551 & .509 & .546 & .418 & .338 & .378 & .599 & .540 & .580 & .798 & .753 & .639 & .816 & .770 & .830 & .664 & .583 & .677 \\
	\textbf{MNP}  & .495 & .523 & .603 & .367 & .337 & .405 & .467 & .486 & .576 & .621 & .778 & \first{.765} & .668 & .724 & .822 & .568 & .555 & .709 \\
	\textbf{UFO}  & .579 & .557 & .610 & .432 & .385 & .433 & .545 & .541 & .593 & .742 & .781 & .729 & .842 & .806 & .862 & .701 & .654 & .739 \\
	\textbf{MC}   & .610 & \third{.603} & .600 & \second{.460} & \third{.420} & .434 & \third{.627} & \third{.603} & .615 & .779 & .803 & .630 & \third{.847} & .824 & .855 & \second{.742} & .704 & .745 \\
	\textbf{DSR}  & \third{.611} & \second{.604} & .597 & .454 & \second{.421} & .410 & .626 & \first{.614} & .593 & .794 & \third{.821} & .632 & .835 & \third{.824} & .833 & .737 & \second{.717} & .703 \\
	\textbf{CHM}  & \second{.612} & .591 & .643 & .417 & .368 & .424 & .604 & .586 & .637 & .750 & .750 & .658 & .825 & .804 & .857 & .722 & .684 & .735 \\
	\textbf{GC}   & .533 & .517 & .497 & .384 & .321 & .342 & .535 & .528 & .506 & .729 & .730 & .616 & .794 & .777 & .780 & .641 & .612 & .593 \\
	\textbf{LBI}  & .519 & .534 & .618 & .371 & .353 & .416 & .482 & .504 & .609 & .692 & .776 & \second{.764} & .696 & .714 & .857 & .586 & .563 & .738 \\
	\textbf{PCA}  & .544 & .558 & .601 & .432 & .404 & .368 & .554 & .554 & .624 & .754 & .796 & .701 & .782 & .782 & .845 & .646 & .627 & .720 \\
	\textbf{DRFI} & \first{.670} & \first{.607} & \first{.674} & \first{.475} & .419 & .447 & \first{.665} & \second{.605} & \first{.669} & \second{.831} & \first{.839} & .702 & \first{.881} & \first{.838} & \first{.905} & \first{.787} & \first{.733} & \first{.801} \\
	\textbf{GMR}  & .597 & .594 & .579 & .454 & .409 & .432 & .610 & .591 & .591 & .773 & .789 & .643 & .847 & \second{.825} & .839 & .740 & \third{.712} & .736 \\
	\textbf{HS}   & .585 & .549 & .602 & .442 & .358 & .428 & .616 & .565 & .616 & .811 & .776 & .713 & .845 & .800 & .870 & .731 & .659 & .769 \\
	\textbf{LMLC} & .540 & .519 & .588 & .375 & .302 & .397 & .521 & .493 & .551 & .653 & .712 & .674 & .801 & .772 & .860 & .659 & .600 & .735 \\
	\textbf{SF}   & .500 & .495 & .342 & .373 & .319 & .219 & .519 & .512 & .377 & .764 & .794 & .509 & .779 & .759 & .573 & .619 & .576 & .378 \\
	\textbf{FES}  & .547 & .575 & .426 & .424 & .411 & .333 & .520 & .555 & .380 & .617 & .785 & .174 & .717 & .753 & .534 & .645 & .655 & .467 \\
	\textbf{CB}   & .581 & .556 & .615 & .444 & .375 & .435 & .542 & .534 & .593 & .730 & .704 & .657 & .815 & .775 & .857 & .717 & .656 & .761 \\
	\textbf{SVO}  & .554 & .441 & .609 & .414 & .279 & .419 & .557 & .407 & .609 & .744 & .667 & .746 & .789 & .585 & .863 & .639 & .357 & .737 \\
	\textbf{SWD}  & .528 & .560 & \third{.649} & .434 & .386 & \third{.454} & .478 & .506 & .613 & .548 & .714 & .737 & .689 & .705 & .871 & .624 & .549 & \second{.781} \\
	\textbf{HC}   & .386 & .401 & .436 & .286 & .257 & .280 & .382 & .380 & .435 & .736 & .759 & .646 & .677 & .663 & .740 & .460 & .441 & .499 \\
	\textbf{RC}   & .610 & .586 & .639 & .431 & .370 & .425 & .599 & .578 & .621 & .774 & .807 & .649 & .844 & .820 & .875 & \third{.741} & .701 & \third{.776} \\
	\textbf{SEG}  & .500 & .425 & .580 & .376 & .268 & .393 & .516 & .450 & .562 & .704 & .640 & .669 & .697 & .585 & .812 & .568 & .408 & .715 \\
	\textbf{MSS}  & .478 & .490 & .200 & .341 & .324 & .089 & .476 & .490 & .193 & .743 & .783 & .298 & .696 & .711 & .362 & .530 & .536 & .203 \\
	\textbf{CA}   & .458 & .494 & .557 & .353 & .330 & .394 & .435 & .458 & .532 & .591 & .737 & .565 & .621 & .679 & .748 & .515 & .494 & .625 \\
	\textbf{FT}   & .386 & .400 & .238 & .278 & .250 & .132 & .381 & .388 & .259 & .715 & .734 & .436 & .635 & .628 & .472 & .434 & .431 & .257 \\
	\textbf{AC}   & .410 & .431 & .068 & .227 & .199 & .049 & .354 & .383 & .040 & .684 & .729 & .140 & .520 & .566 & .014 & .411 & .410 & .038 \\
	\textbf{LC}   & .386 & .408 & .289 & .264 & .246 & .156 & .327 & .353 & .243 & .683 & .752 & .486 & .569 & .589 & .432 & .390 & .396 & .219 \\
	\hline \hline
	\textbf{OBJ}  & .498 & .482 & .593 & .368 & .282 & .413 & .481 & .445 & .578 & .685 & .723 & .731 & .718 & .681 & .840 & .574 & .456 & .698 \\
	\hline \hline
	\textbf{BMS}  & .568 & .578 & .594 & .434 & .404 & .416 & .573 & .576 & .580 & .713 & .760 & .627 & .805 & .798 & .822 & .683 & .659 & .690 \\
	\textbf{COV}  & .510 & .587 & .398 & .429 & \first{.427} & .315 & .486 & .579 & .373 & .518 & .724 & .212 & .667 & .755 & .394 & .641 & .677 & .413 \\
	\textbf{SS}   & .415 & .482 & .523 & .344 & .321 & .397 & .396 & .443 & .502 & .533 & .696 & .641 & .572 & .642 & .675 & .467 & .441 & .574 \\
	\textbf{SIM}  & .372 & .429 & .568 & .295 & .292 & .384 & .358 & .402 & .539 & .498 & .685 & .725 & .498 & .585 & .794 & .433 & .391 & .672 \\
	\textbf{SeR}  & .374 & .419 & .536 & .316 & .285 & .388 & .385 & .411 & .532 & .521 & .714 & .702 & .542 & .607 & .755 & .419 & .391 & .596 \\
	\textbf{SUN}  & .387 & .432 & .486 & .303 & .291 & .285 & .321 & .360 & .445 & .504 & .661 & .613 & .505 & .596 & .670 & .388 & .376 & .478 \\
	\textbf{SR}   & .374 & .457 & .002 & .279 & .270 & .001 & .298 & .363 & .000 & .504 & .700 & .002 & .473 & .569 & .001 & .381 & .385 & .001 \\
	\textbf{GB}   & .526 & .571 & \second{.650} & .419 & .396 & \second{.455} & .507 & .548 & .638 & .571 & .746 & .695 & .688 & .737 & .837 & .624 & .613 & .765 \\
	\textbf{AIM}  & .427 & .461 & .559 & .317 & .260 & .360 & .361 & .377 & .495 & .541 & .718 & .693 & .555 & .575 & .750 & .449 & .357 & .571 \\
	\textbf{IT}   & .373 & .437 & .005 & .297 & .283 & .000 & .378 & .449 & .005 & .579 & .697 & .008 & .471 & .586 & .158 & .407 & .414 & .003 \\
	\hline \hline
	\textbf{AAM}  & .458 & .569 & .620 & .392 & .367 & .411 & .406 & .514 & .534 & .388 & .524 & .640 & .580 & .692 & .779 & .597 & .627 & .756 \\
\hline
\end{tabular}


==> Results/MAE.tex <==
\begin{tabular}{|l||c|c|c|c|c|c|} \hline
	\tabTitle \\	\hline \hline
	\textbf{HDCT} & .177 & .209 & .164 & .162 & .143 & .199 \\
	\textbf{RBD}  & \third{.150} & .212 & \second{.144} & \second{.130} & \first{.108} & \third{.173} \\
	\textbf{GR}   & .256 & .311 & .259 & .189 & .198 & .285 \\
	\textbf{MNP}  & .255 & .286 & .272 & .215 & .229 & .307 \\
	\textbf{UFO}  & .165 & .216 & .173 & .180 & .150 & .207 \\
	\textbf{MC}   & .184 & .231 & .186 & .182 & .145 & .204 \\
	\textbf{DSR}  & \first{.142} & .196 & \first{.139} & \third{.140} & \third{.121} & \second{.173} \\
	\textbf{CHM}  & .153 & .226 & \third{.152} & .168 & .142 & .195 \\
	\textbf{GC}   & .192 & .258 & .197 & .185 & .139 & .214 \\
	\textbf{LBI}  & .239 & .273 & .249 & .207 & .224 & .280 \\
	\textbf{PCA}  & .198 & \first{.181} & .206 & .200 & .185 & .248 \\
	\textbf{DRFI} & \second{.150} & .213 & .155 & \first{.130} & \second{.118} & \first{.166} \\
	\textbf{GMR}  & .181 & .243 & .189 & .163 & .126 & .189 \\
	\textbf{HS}   & .218 & .282 & .227 & .157 & .149 & .228 \\
	\textbf{LMLC} & .246 & .303 & .277 & .269 & .163 & .260 \\
	\textbf{SF}   & .184 & .218 & .183 & .180 & .175 & .230 \\
	\textbf{FES}  & .155 & \third{.184} & .156 & .196 & .185 & .215 \\
	\textbf{CB}   & .227 & .287 & .257 & .195 & .178 & .241 \\
	\textbf{SVO}  & .382 & .422 & .409 & .348 & .331 & .404 \\
	\textbf{SWD}  & .288 & .292 & .310 & .296 & .267 & .318 \\
	\textbf{HC}   & .291 & .348 & .310 & .193 & .215 & .331 \\
	\textbf{RC}   & .168 & .270 & .189 & .148 & .137 & .187 \\
	\textbf{SEG}  & .336 & .354 & .337 & .312 & .298 & .342 \\
	\textbf{MSS}  & .178 & .204 & .177 & .192 & .203 & .245 \\
	\textbf{CA}   & .248 & .282 & .254 & .229 & .237 & .310 \\
	\textbf{FT}   & .241 & .267 & .250 & .206 & .235 & .291 \\
	\textbf{AC}   & .186 & .239 & .190 & .206 & .227 & .265 \\
	\textbf{LC}   & .229 & .277 & .246 & .204 & .233 & .296 \\
	\hline \hline
	\textbf{OBJ}  & .306 & .359 & .323 & .269 & .262 & .337 \\
	\hline \hline
	\textbf{BMS}  & .181 & .233 & .175 & .184 & .151 & .216 \\
	\textbf{COV}  & .155 & \second{.182} & .156 & .210 & .197 & .217 \\
	\textbf{SS}   & .267 & .301 & .277 & .266 & .266 & .344 \\
	\textbf{SIM}  & .414 & .412 & .429 & .384 & .388 & .433 \\
	\textbf{SeR}  & .345 & .379 & .352 & .290 & .310 & .404 \\
	\textbf{SUN}  & .310 & .319 & .349 & .307 & .306 & .396 \\
	\textbf{SR}   & .175 & .200 & .181 & .220 & .232 & .266 \\
	\textbf{GB}   & .229 & .261 & .240 & .242 & .222 & .263 \\
	\textbf{AIM}  & .298 & .331 & .322 & .262 & .286 & .339 \\
	\textbf{IT}   & .199 & .200 & .198 & .245 & .213 & .273 \\
	\hline \hline
	\textbf{AAM}  & .248 & .343 & .288 & .405 & .260 & .276 \\
\hline
\end{tabular}


==> Results/MaxAdpScTUnCentered.tex <==
\renewcommand{\tabcolsep}{.56mm}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method & HDCT&  RBD&   GR&  MNP&  UFO&   MC&  DSR&  CHM&   GC&  LBI&  PCA& DRFI&  GMR&   HS& LMLC&   SF&  FES&   CB&  SVO \\\hline
	Max   & \second{.822} & .811 & .791 & .661 & .805 & .764 & .776 & .746 & .697 & .685 & .750 & \first{.831} & .754 & \third{.815} & .720 & .747 & .621 & .693 & .792  \\
	AUC   & .941 & \second{.943} & .925 & .912 & .929 & .888 & .938 & .920 & .860 & .910 & .928 & \first{.964} & .886 & .918 & .896 & .885 & .839 & .872 & \third{.942}  \\
	MAE   & \third{.122} & \first{.106} & .183 & .188 & .128 & .171 & \second{.117} & .138 & .164 & .197 & .162 & .127 & .148 & .150 & .201 & .150 & .160 & .207 & .325  \\
\hline
\end{tabular}
\renewcommand{\tabcolsep}{.425mm}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method & SWD &  HC&   RC&  SEG&  MSS&   CA&   FT&   AC&   LC&  OBJ&  BMS&  COV&   SS&  SIM&  SeR&  SUN&   SR&   GB&  AIM&   IT&  AAM\\\hline
	Max   & .521 & .700 & .744 & .629 & .666 & .620 & .671 & .521 & .569 & .708 & .739 & .463 & .571 & .515 & .546 & .498 & .444 & .590 & .540 & .460 & .328 \\
	AUC   & .813 & .898 & .855 & .828 & .868 & .896 & .843 & .800 & .797 & .915 & .879 & .805 & .852 & .858 & .849 & .795 & .750 & .850 & .836 & .655 & .716 \\
	MAE   & .291 & .176 & .177 & .300 & .167 & .199 & .183 & .177 & .192 & .243 & .146 & .176 & .225 & .363 & .273 & .276 & .184 & .208 & .265 & .165 & .406 \\
\hline
\end{tabular}


==> Results/MaxFRnk.tex <==
\renewcommand{\tabcolsep}{1.51mm}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method & HDCT&  RBD&   GR&  MNP&  UFO&   MC&  DSR&  CHM&   GC&  LBI&  PCA& DRFI&  GMR&   HS& LMLC&   SF&  FES&   CB&  SVO\\\hline
	$F_\beta$& 8 & \third{3} & 10 & 27 & 11 & \second{2} & 4 & 9 & 16 & 23 & 14 & \first{1} & 5 & 6 & 17 & 19 & 18 & 12 & 15 \\
	%Mean  & 8 & \third{3} & 13 & 19 & 14 & 6 & \first{1} & 10 & 9 & 17 & 16 & \second{2} & 4 & 5 & 15 & 20 & 26 & 12 & 18 \\
	AUC   & 7 & \third{3} & 21 & 20 & 16 & 4 & \second{2} & 6 & 28 & 13 & 5 & \first{1} & 9 & 12 & 23 & 26 & 18 & 19 & 11 \\
	MAE   & 5 & \second{2} & 26 & 28 & 6 & 11 & \first{1} & 4 & 15 & 23 & 16 & \third{3} & 9 & 17 & 27 & 13 & 8 & 21 & 39 \\
	AdpT  & 7 & 5 & 17 & 21 & 13 & \third{3} & \second{2} & 8 & 19 & 20 & 12 & \first{1} & 4 & 14 & 25 & 18 & 11 & 16 & 37 \\
	SCut  & 4 & \second{2} & 24 & 14 & 8 & 13 & 20 & 11 & 29 & 9 & 15 & \first{1} & 17 & 7 & 18 & 33 & 32 & 12 & 10  \\
	CB    & \second{2} & 4 & 7 & 24 & 5 & 9 & 8 & 13 & 19 & 21 & 11 & \first{1} & 10 & \third{3} & 16 & 12 & 26 & 20 & 6 \\
	Time  & 27 & 15 & 23 & 34 & 33 & 13 & 30 & 32 & \third{3} & 39 & 28 & 19 & 11 & 17 & 38 & 14 & 8 & 24 & 37  \\
\hline
\hline
\end{tabular}
\renewcommand{\tabcolsep}{1.4185mm}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
	Method&  SWD &   HC&   RC&  SEG&  MSS&   CA&   FT&   AC&   LC&  OBJ&  \textbf{BMS}&  \textbf{COV}&   \textbf{SS}&  \textbf{SIM}&  \textbf{SeR}&  \textbf{SUN}&   \textbf{SR}&   \textbf{GB}&  \textbf{AIM}&   \textbf{IT}& AAM\\\hline
	$F_\beta$& 20 & 30 & 7 & 22 & 26 & 28 & 32 & 34 & 36 & 25 & 13 & 24 & 31 & 39 & 35 & 38 & 40 & 21 & 33 & 37 & 29 \\
	%Mean  & 25 & 23 & 7 & 21 & 34 & 28 & 33 & 38 & 31 & 22 & 11 & 30 & 32 & 36 & 29 & 37 & 40 & 24 & 35 & 39 & 27 \\
	AUC   & 17 & 31 & 8 & 29 & 27 & 24 & 37 & 35 & 39 & 22 & 14 & 10 & 32 & 33 & 34 & 36 & 38 & 15 & 30 & 40 & 25 \\
	MAE   & 33 & 30 & 7 & 37 & 14 & 29 & 25 & 19 & 24 & 35 & 12 & 10 & 32 & 40 & 38 & 36 & 18 & 22 & 34 & 20 & 31 \\
	AdpT  & 22 & 29 & 6 & 36 & 24 & 26 & 32 & 35 & 33 & 27 & 9 & 10 & 28 & 34 & 31 & 39 & 40 & 15 & 38 & 30 & 23 \\
	SCut  & \third{3}& 30 & 6 & 22 & 37 & 27 & 35 & 38 & 36 & 16 & 21 & 34 & 28 & 23 & 25 & 31 & 40 & 5 & 26 & 39 & 19 \\
	CB    & 34 & 18 & 14 & 25 & 23 & 27 & 22 & 33 & 30 & 17 & 15 & 37 & 29 & 35 & 31 & 36 & 39 & 28 & 32 & 38 & 40 \\
	Time  & 12 & \second{2} & 10 & 31 & 7 & 36 & 6 & 9 & \first{1} & 25 & 18 & 35 & 5 & 21 & 22 & 26 & 4 & 20 & 29 & 16 & 40 \\
\hline
\end{tabular}

